Self-consistent gyrokinetic modelling of turbulent and neoclassical tungsten transport in toroidally rotating plasmas

The effect of toroidal rotation on both turbulent and neoclassical transport of tungsten (W) in tokamaks is investigated using the flux-driven, global, nonlinear 5D gyrokinetic code GYSELA. Nonlinear simulations are carried out with different levels of momentum injection that drive W to the supersonic regime, while the toroidal velocity of the main ions remains in the subsonic regime. The numerical simulations demonstrate that toroidal rotation induces centrifugal forces that cause W to accumulate in the outboard region, generating an in-out poloidal asymmetry. This asymmetry enhances neoclassical inward convection, which can lead to central accumulation of W in cases of strong plasma rotation. The core accumulation of W is mainly driven by inward neoclassical convection. However, as momentum injection continues, roto-diffusion, proportional to the radial gradient of the toroidal velocity, becomes significant and generate outward turbulent flux in the case of ion temperature gradient (ITG) turbulence. Overall, the numerical results from nonlinear GYSELA simulations are in qualitative agreement with the theoretical predictions for impurity transport, as well as experimental observations.

==> 9_bib.tex <==
@article{Casson2010,
    author = {Casson, F.J. and others},
    title = {Gyrokinetic simulations including the centrifugal force in a rotating tokamak plasma},
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/1.3491110}
    {\textbf{17} 102305}},
    year = {(2010)},
}

@article{Wong1987_b,
    author = {Wong, K. L. and Cheng, C. Z.},
    title = {Neoclassical Diffusion of Heavy Impurities in a Rotating Tokamak Plasma},
    journal = {Phys. Rev. Lett.},
    volume =  {\href{https://doi.org/10.1103/PhysRevLett.59.2643}
    {\textbf{59} 2643}},
    year = {(1987)},
}

@article{Camenen2009,
    author = {Camenen,Y. and Peeters,A. G.  and Angioni,C.  and Casson,F. J.  and Hornsby,W. A.  and Snodin,A. P.  and Strintzi,D. },
    title = {Impact of the background toroidal rotation on particle and heat turbulent transport in tokamak plasmas},
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/1.3057356}
    {\textbf{16} 012503}},
    year = {(2009)},
}

@article{Goniche2017,
    author = {Goniche, M. and others},
    title = {{Ion cyclotron resonance heating for tungsten control in various JET H-mode scenarios}},
    journal = {Plasma Phys. Control. Fusion},
    volume =  {\href{https://doi.org/10.1088/1361-6587/aa60d2}
    {\textbf{59} 055001}},
    year = {(2017)},
}

@article{Rice2007,
    author = {Rice, J. E. and others},
    title = {Inter-machine comparison of intrinsic toroidal rotation in tokamaks},
    journal = {Nucl. Fusion},
    volume =  {\href{https://doi.org/10.1088/0029-5515/47/11/025}
    {\textbf{47} 1618}},
    year = {(2007)},
}

@article{Peeters2009,
    author = {Peeters, A. G. and others},
    title = {Influence of the centrifugal force and parallel dynamics on the toroidal momentum transport due to small scale turbulence in a tokamak},
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/1.3097263}
    {\textbf{16} 042310}},
    year = {(2009)},
}

@article{Wesson1997,
    author = {Wesson, J.A.},
    title = {Poloidal distribution of impurities in a rotating tokamak plasma},
    journal = {Nucl. Fusion},
    volume =  {\href{https://doi.org/10.1088/0029-5515/37/5/I01}
    {\textbf{37} 577}},
    year = {(1997)},
}

@article{Bortolon2006,
    author = {Bortolon, A. and others},
    title = {Observation of Spontaneous Toroidal Rotation Inversion in Ohmically Heated Tokamak Plasmas},
    journal = {Phys. Rev. Lett.},
    volume =  {\href{https://doi.org/10.1103/PhysRevLett.97.235003}
    {\textbf{97} 235003}},
    year = {(2006)},
}

@article{Romanelli1998,
    author = {Romanelli, M. and Ottaviani, M},
    title = {Effects of density asymmetries on heavy impurity transport in a rotating tokamak plasma},
    journal = {Plasma Phys. Control. Fusion},
    volume =  {\href{https://doi.org/10.1088/0741-3335/40/10/007}
    {\textbf{40} 1767}},
    year = {(1998)},
}

@article{Fulop1999,
    author = {Fülöp, T. and Helander, P},
    title = {Nonlinear neoclassical transport in a rotating impure plasma with large gradients},
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/1.873593}
    {\textbf{6} 3066}},
    year = {(1999)},
}

@article{Catto1987,
    author = {Catto, P. J. and Bernstein, I. B. and Tessarotto, M.},
    title = {Ion transport in toroidally rotating tokamak plasmas},
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/1.866045}
    {\textbf{30} 2784}},
    year = {(1987)},
}

@article{Wong1982,
    author = {Wong, S. K. and Burrell, K. H.},
    title = {Transport theory of tokamak plasmas with large toroidal rotation},
    journal = {Phys. Fluids},
    volume =  {\href{https://doi.org/10.1063/1.863665}
    {\textbf{25} 1863}},
    year = {(1982)},
}

@article{Wong1987,
    author = {Wong, S. K.},
    title = {Transport of impure plasma with arbitrary toroidal rotation},
    journal = {Phys. Fluids},
    volume =  {\href{https://doi.org/10.1063/1.866333}
    {\textbf{30} 818}},
    year = {(1987)},
}

@article{Hinton1985,
    author = {Hinton, F. L. and Wong, S. K.},
    title = {Neoclassical ion transport in rotating axisymmetric plasmas},
    journal = {Phys. Fluids},
    volume =  {\href{https://doi.org/10.1063/1.865350}
    {\textbf{28} 3082}},
    year = {(1985)},
}

@article{Helander1998,
    author = {Helander, P.},
    title = {Neoclassical transport in a rotating impure plasma},
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/1.872629}
    {\textbf{5} 1209}},
    year = {(1998)},
}

@article{Sugama2017,
    author = {Sugama, H.},
    title = {Modern gyrokinetic formulation of collisional and turbulent transport in toroidally rotating plasmas},
    journal = {Rev. Mod. Plasma Phys.},
    volume =  {\href{https://doi.org/10.1007/s41614-017-0010-5}
    {\textbf{1} 9}},
    year = {(2017)},
}

@article{Belli2014,
    author = {Belli, E. A. and Candy, J. and Angioni, C.},
    title = {Pfirsch–Schlüter neoclassical heavy impurity transport in a rotating plasma},
    journal = {Plasma Phys. Control. Fusion},
    volume =  {\href{https://doi.org/10.1088/0741-3335/56/12/124002}
    {\textbf{56} 124002}},
    year = {(2014)},
}

@article{Bilato2014,
    author = {Bilato, R. and Maj, O. and Angioni, C.},
    title = {Modelling the influence of temperature anisotropies on poloidal asymmetries of density in the core of rotating plasmas},
    journal = {Nucl. Fusion},
    volume =  {\href{https://doi.org/10.1088/0029-5515/54/7/072003}
    {\textbf{54} 072003}},
    year = {(2014)},
}

@article{Sugama1997,
    author = {Sugama, H. and Horton, W.},
    title = {Neoclassical electron and ion transport in toroidally rotating plasmas},
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/1.872385}
    {\textbf{4} 2215}},
    year = {(1997)},
}

@article{Choe1995,
    author = {Choe, W. and Chang, C. S. and Ono, M.},
    title = {Temperature anisotropy in a cyclotron resonance heated tokamak plasma and the generation of poloidal electric field},
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/1.871456}
    {\textbf{2} 2044}},
    year = {(1995)},
}

@article{Brizard1995,
    author = {Brizard, A. J.},
    title = {{Nonlinear gyrokinetic Vlasov equation for toroidally rotating axisymmetric tokamaks}},
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/1.871465}
    {\textbf{2} 459}},
    year = {(1995)},
}

@article{Angioni2014,
    author = {Angioni, C. and Helander, P.},
    title = {Neoclassical transport of heavy impurities with poloidally asymmetric density distribution in tokamaks},
    journal = {Plasma Phys. Control. Fusion},
    volume =  {\href{https://doi.org/10.1088/0741-3335/56/12/124001}
    {\textbf{56} 124001}},
    year = {(2014)},
}

@article{Bilato2017,
    author = {Bilato, R. and others},
    title = {The impact of the ion-cyclotron-resonance location on the poloidal asymmetries of impurity density in an {ICRF}-heated rotating plasma},
    journal = {Nucl. Fusion},
    volume =  {\href{https://doi.org/10.1088/1741-4326/aa5fd6}
    {\textbf{57} 056020}},
    year = {(2017)},
}

@article{Hahm1992,
    author = {Hahm, T. S.},
    title = {Trapped particle dynamics in toroidally rotating plasmas},
    journal = {Phys. Fluids B},
    volume =  {\href{https://doi.org/10.1063/1.860310}
    {\textbf{4} 4046}},
    year = {(1992)},
}

@article{Reinke2013,
    author = {Reinke, M. L. and others},
    title = {{Parallel transport studies of high-{Z} impurities in the core of {A}lcator {C}-{M}od plasmas}},
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/1.4802197}
    {\textbf{20} 056109}},
    year = {(2013)},
}

@article{Hirshman1981,
    author = {Hirshman, S. P. and Sigmar, D. J.},
    title = {Neoclassical transport of impurities in tokamak plasmas},
    journal = {Nucl. Fusion},
    volume =  {\href{https://doi.org/10.1088/0029-5515/21/9/003}
    {\textbf{21} 1079}},
    year = {(1981)},
}

@article{Hinton1999,
    author = {Hinton, F. L. and Rosenbluth, M. N.},
    title = {Dynamics of axisymmetric ${E} \times {B}$  and poloidal flows in tokamaks},
    journal = {Plasma Phys. Control. Fusion},
    volume =  {\href{https://doi.org/10.1088/0741-3335/41/3A/059}
    {\textbf{41} A653}},
    year = {(1999)},
}

@article{Sarazin2011,
    author = {Sarazin, Y. and others},
    title = {Predictions on heat transport and plasma rotation from global gyrokinetic simulations},
    journal = {Nucl. Fusion},
    volume =  {\href{https://doi.org/10.1088/0029-5515/51/10/103023}
    {\textbf{51} 103023}},
    year = {(2011)},
}

@article{Putterich2010,
    author = {T. Pütterich and R. Neu and R. Dux and A.D. Whiteford and M.G. O'Mullane and H.P. Summers and the ASDEX Upgrade Team},    
    title = {Calculation and experimental test of the cooling factor of tungsten},
    journal = {Nucl. Fusion},
    volume = {\href{https://doi.org/10.1088/0029-5515/50/2/025012}
    {\textbf{50} 025012}},
    year = {(2016)},
}

@article{Maget2020,
    author = {Maget, P. and others},
    title = {Natural poloidal asymmetry and neoclassical transport of impurities in tokamak plasmas},
    journal = {Plasma Phys. Control. Fusion},
    volume = {\href{https://doi.org/10.1088/1361-6587/ab53ab}
    {\textbf{62} 025001}},
    year = {(2020)},
}

@article{Casson2013,
    author = {Casson, F. J. and others},
    title = {Validation of gyrokinetic modelling of light impurity transport including rotation in {ASDEX} {U}pgrade},
    journal = {Nucl. Fusion},
    volume = {\href{https://doi.org/10.1088/0029-5515/53/6/063026}
    {\textbf{53} 063026}},
    year = {(2013)},
}

@article{Casson2015,
    author = {Casson, F. J. and others},
    title = {Theoretical description of heavy impurity transport and its application to the modelling of tungsten in {JET} and {ASDEX} upgrade},
    journal = {Plasma Phys. Control. Fusion},
    volume = {\href{https://doi.org/10.1088/0741-3335/57/1/014031}
    {\textbf{57} 014031}},
    year = {(2015)},
}

@article{Angioni2014_2,
    author = {Angioni, C. and others},
    title = {{Tungsten transport in {JET} {H}-mode plasmas in hybrid scenario, experimental observations and modelling}},
    journal = {Nucl. Fusion},
    volume = {\href{https://doi.org/10.1088/0029-5515/54/8/083028}
    {\textbf{54} 083028}},
    year = {(2014)},
}

@article{Lim2020,
    author = {Lim, K. and others},
    title = {Impurity pinch generated by trapped particle driven turbulence},
    journal = {Plasma Phys. Control. Fusion},
    volume = {\href{https://doi.org/10.1088/1361-6587/aba340}
    {\textbf{62} 095018}},
    year = {(2020)},
}

@article{Lim2021,
    author = {Lim, K. and others},
    title = {Gyrokinetic modelling of light to heavy impurity transport in tokamaks},
    journal = {Nucl. Fusion},
    volume = {\href{https://doi.org/10.1088/1741-4326/abe6b4}
    {\textbf{61} 046037}},
    year = {(2021)},
}

@article{Stacey1985,
    author = {W.M. Stacey and A.W. Bailey and D.J. Sigmar and K.C. Shaing},
    title = {Rotation and impurity transport in a tokamak plasma with directed neutral-beam injection},
    journal = {Nucl. Fusion},
    volume = {\href{https://doi.org/10.1088/0029-5515/25/4/007}
    {\textbf{25} 463}},
    year = {(1985)},
}

@article{Stacey1992,
    author = {W.M. Stacey},
    title = {Poloidal rotation and density asymmetries in a tokamak plasma with strong toroidal rotation},
    journal = {Phys. Fluids B},
    volume = {\href{https://doi.org/10.1063/1.860476}
    {\textbf{4} 3302}},
    year = {1992},
}

@article{Burrell1981,
    author = {Burrell, K.H. and Ohkawa, T. and Wong, S. K.},
    title = {Explanation of the Expulsion of Impurities from Tokamak Plasmas by Neutral-Beam Injection},
    journal = {Phys. Rev. Lett.},
    volume = {\href{https://doi.org/10.1103/PhysRevLett.47.511}
    {\textbf{47} 511}},
    year = {(1981)},
}

@article{Gravier2019,
    author = {Gravier, E. and others},
    title = {Diffusive impurity transport driven by trapped particle turbulence in tokamak plasmas},
    journal = {Phys. Plasmas},
    volume = {\href{https://doi.org/10.1063/1.5107443}
    {\textbf{26} 082306}},
    year = {(2019)},
}

@article{Lesur2020,
    author = {Lesur, M. and others},
    title = {Validity limits of the passive treatment of impurities in gyrokinetic tokamak simulations},
    journal = {Nucl. Fusion},
    volume = {\href{https://doi.org/10.1088/1741-4326/ab6e48}
    {\textbf{60} 036016}},
    year = {(2020)},
}

@article{Angioni2012_a,
    author = {Angioni, C. and others},
    title = {Analytic formulae for centrifugal effects on turbulent transport of trace impurities in tokamak plasmas},
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/1.4773051}
    {\textbf{19} 122311}},
    year = {(2012)},
}

@article{Angioni2015,
    author = {Angioni, C. and others},
    title = {The impact of poloidal asymmetries on tungsten transport in the core of {JET} {H}-mode plasmas},
    journal = {Phys. Plasmas},
    volume = {\href{https://doi.org/10.1063/1.4919036}
    {\textbf{22} 055902}},
    year = {(2015)},
}

@article{Vries2008,
    author = {de Vries, P. C. and others},
    title = {Scaling of rotation and momentum confinement in {JET} plasmas},
    journal = {Nucl. Fusion},
    volume =  {\href{https://doi.org/10.1088/0029-5515/48/6/065006}
    {\textbf{48} 065006}},
    year = {(2008)},
}

@article{Donnel2019_b,
    author = {Donnel, P. and others},
    title = {Turbulent generation of poloidal asymmetries of the electric potential in a tokamak},
    journal = {Plasma Phys. Control. Fusion},
    volume = {\href{https://doi.org/10.1088/1361-6587/ab04b8}
    {\textbf{61} 044006}},
    year = {(2019)},
}

@article{Casson2020,
    author = {Casson, F. J. and others},
    title = {{Predictive multi-channel flux-driven modelling to optimise {ICRH} tungsten control and fusion performance in {JET}}},
    journal = {Nucl. Fusion},
    volume = {\href{https://doi.org/10.1088/1741-4326/ab833f}
    {\textbf{60} 066209}},
    year = {(2020)},
}

@article{Wong1989,
    author = {Wong, K. L. and Cheng, C. Z.},
    title = {Orbit effects on impurity transport in a rotating tokamak plasma},
    journal = {Phys. Fluids B},
    volume = {\href{https://doi.org/10.1063/1.859170}
    {\textbf{1} 545}},
    year = {(1989)},
}

@article{Angioni2017,
    author = {Angioni, C. and others},
    title = {{A comparison of the impact of central ECRH and central ICRH on the tungsten behaviour in ASDEX Upgrade H-mode plasmas}},
    journal = {Nucl. Fusion},
    volume = {\href{https://doi.org/10.1088/1741-4326/aa6453}
    {\textbf{57} 056015}},
    year = {(2017)},
}

@article{Kim1991,
    author = {Kim,Y. B.  and Diamond, P. H. and Groebner,R. J. },
    title = {Neoclassical poloidal and toroidal rotation in tokamaks},
    journal = {Phys. Fluids B},
    volume = {\href{https://doi.org/10.1063/1.859671}
    {\textbf{3} 2050}},
    year = {(1991)},
}

@book{Rice2022,
    author    = {J. Rice},
    title     = {{Driven Rotation, Self-Generated Flow, and Momentum Transport in Tokamak Plasmas}},
    year      = {(2022)},
    publisher = {Springer Cham},
    address   = {London}
}

@article{Ida2014,
	author = {K. Ida and J.E. Rice},
	title = {Rotation and momentum transport in tokamaks and helical systems},
	journal = {Nucl. Fusion},
	volume = {\href{https://doi.org/10.1088/0029-5515/54/4/045001}{\textbf{54} 045001}},
	year = {(2014)},
}

@article{Eriksson1997,
    author = {L. G. Eriksson and E. Righi and K. D. Zastrow},
    title = {{Toroidal rotation in {ICRF}-heated H-modes on {JET}}},
    journal = {Plasma Phys. Control. Fusion},
    volume = {\href{https://doi.org/10.1088/0741-3335/39/1/002}{\textbf{39} 27}},
    year = {(1997)},
}

@article{Callen2009,
    author = {Callen,J. D.  and Cole,A. J.  and Hegna,C. C. },
    title = {Toroidal flow and radial particle flux in tokamak plasmas},
    journal = {Phys. Plasmas},
    volume = {\href{https://doi.org/10.1063/1.3206976}{\textbf{16} 082504}},
    year = {(2009)},
}


@article{Scott10,
    author = "Scott, B. and Smirnov, J.",
    title = "Energetic consistency and momentum conservation in the gyrokinetic description of tokamak plasmas",
    journal = "Phys. Plasmas",
    volume = "\href{https://doi.org/10.1063/1.3507920}
    {\textbf{17} 112302}",
    year = "2010",
}

@article{Wong2008,
    author = {Wong,S. K. and Chan,V. S.  and Solomon,W. M. },
    title = {Poloidal velocity of impurity ions in neoclassical theory},
    journal = {Phys. Plasmas},
    volume =       {\href{https://doi.org/10.1063/1.2969438}
    {\textbf{15} 082503}},
    year = {(2008)},
}

@article{Newton2006,
    author = {Newton,S.  and Helander,P. },
    title = {Neoclassical momentum transport in an impure rotating tokamak plasma},
    journal = {Phys. Plasmas},
    volume =       {\href{https://doi.org/10.1063/1.2160518}
    {\textbf{13} 012505}},
    year = {(2006)},
}

@article{Hinton1976,
    title = {Theory of plasma transport in toroidal confinement systems},
    author = {Hinton, F. L. and Hazeltine, R. D.},
    journal = {Rev. Mod. Phys.},
    volume =       {\href{https://doi.org/10.1103/RevModPhys.48.239}{\textbf{48} 239}},
    year = {(1976)},
}


@article{Bae2014,
    author = {Bae, C. and  Stacey, W. M. and Lee, S. G.  and Terzolo,L. },
    title = {{Predictions of the poloidal asymmetries and transport frequencies in KSTAR}},
    journal = {Phys. Plasmas},
    volume =       {\href{https://doi.org/10.1063/1.4848175}{\textbf{21} 012504}},
    year = {(2014)},
}

@article{Grandgirard2016,
    author = {Grandgirard, V. and others},
    title = {A 5{D} gyrokinetic full-{F} global semi-Lagrangian code for flux-driven ion turbulence simulations},
    journal = {Comp. Phys. Comm.},
    volume = {\href{https://doi.org/10.1016/j.cpc.2016.05.007}
    {\textbf{207} 35}},
    year = {(2016)},
}

@article{Lo-Cascio2022,
    author = {G. Lo-Cascio and others},
    title = {{Transport barrier in 5D gyrokinetic flux-driven simulations}},
    journal = {Nucl. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/1741-4326/ac945d}
    {\textbf{62} 126026}},
    year = {(2022)},
}

@article{Garofalo2009,
    author = {A. M. Garofalo and others},
    title = {Plasma rotation driven by static nonresonant magnetic fields},
    journal = {Phys. Plasmas},
    volume = {\href{ https://doi.org/10.1063/1.3129164}
    {\textbf{16} 056119}},
    year = {(2009)},
}

@article{Hutchinson2000,
  title = {Self-Acceleration of a Tokamak Plasma during Ohmic H Mode},
  author = {I. H. Hutchinson and others},
  journal = {Phys. Rev. Lett.},
  volume = {\href{ https://doi.org/10.1103/PhysRevLett.84.3330}{\textbf{84} 3330}},
  year = {(2000)},
}

@article{Rice2001,
    author = {J.E. Rice and others},
    title = {{Observations of impurity toroidal rotation suppression with ITB formation in ICRF and ohmic H mode Alcator C-Mod plasmas}},
    journal = {Nucl. Fusion},
    volume = {\href{ https://doi.org/10.1088/0029-5515/41/3/304}{\textbf{41} 277}},
    year = {(2001)},
}


@article{Lee2022,
    author = {Lee, H.  and others},
    title = {{Neoclassical transport analysis of high rotational trace limit tungsten impurities in KSTAR tokamak}},
    journal = {Phys. Plasmas},
    volume = {\href{https://doi.org/10.1063/5.0071192}{\textbf{29} 022504}},
    year = {(2022)},
}


@article{Shengyu2022,
    author = {Shengyu Shi and others},
    title = {{Understanding core heavy impurity transport in a hybrid discharge on EAST}},
    journal = {Nucl. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/1741-4326/ac3e3b}{\textbf{62} 066032}},
    year = {(2022)},
}

@article{Pütterich2013,
    pages = {124036},
    author = {T. Pütterich and others},
    title = {{Observations on the W-transport in the core plasma of JET and ASDEX Upgrade}},
    journal = {Plasma Phys. Control. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/0741-3335/55/12/124036}{\textbf{55} 124036}},
    year = {(2013)},
}

@article{Valisa2011,
    author = {M. Valisa and others},
    title = {{Metal impurity transport control in JET H-mode plasmas with central ion cyclotron radiofrequency power injection}},
    journal = {Nucl. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/0029-5515/51/3/033002}{\textbf{51} 033002}},
    year = {(2011)},
}

@article{Puiatti2006,
    author = {Puiatti, M. E.  and others},
    title = {{Analysis of metallic impurity density profiles in low collisionality Joint European Torus H-mode and L-mode plasmas}},
    journal = {Phys. Plasmas},
    volume = {\href{https://dx.doi.org/10.1063/1.2187424}{\textbf{13} 042501}},
    year = {(2011)},
}

@article{Dux2003,
    author = {R. Dux and others},
    title = {{Influence of the heating profile on impurity transport in ASDEX Upgrade}},
    journal = {Plasma Phys. Control. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/0741-3335/45/9/317}{\textbf{45} 1815}},
    year = {(2003)},
}

@article{Tokar1997,
    author = {M.Z. Tokar and others},
    title = {{Nature of high-Z impurity accumulation in tokamaks}},
    journal = {Nucl. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/0029-5515/37/12/I03}{\textbf{37} 1691}},
    year = {(1997)},
}

@article{Odstrcil2018,
    author = {T. Odstrcil and others},
    title = {{The physics of W transport illuminated by recent progress in W density diagnostics at ASDEX Upgrade}},
    journal = {Plasma Phys. Control/ Fusion},
    volume = {\href{https://dx.doi.org/10.1088/1361-6587/aa8690}{\textbf{60} 014003}},
    year = {(2018)},
}

@article{Sertoli2017,
    author = {Sertoli,M.  and Angioni,C.  and Odstrcil,T. },
    title = {{Parametric dependencies of the experimental tungsten transport coefficients in ICRH and ECRH assisted ASDEX Upgrade H-modes}},
    journal = {Phys. Plasmas},
    volume = {\href{https://doi.org/10.1063/1.4996412}{\textbf{24} 112503}},
    year = {(2017)},
}


@article{Breton2018,
    author = {Breton,S.  and others},
    title = {{High Z neoclassical transport: Application and limitation of analytical formulae for modelling JET experimental parameters}},
    journal = {Phys. Plasmas},
    volume = {\href{https://doi.org/10.1063/1.5019275}{\textbf{25} 012303}},
    year = {(2018)},
}



@article{Catto1973,
    author = {Catto, P. J.  and Rosenbluth, M. N.  and Liu,C. S.},
    title = {Parallel velocity shear instabilities in an inhomogeneous plasma with a sheared magnetic field},
    journal = {Phys. Fluids},
    volume = {\href{https://aip.scitation.org/doi/pdf/10.1063/1.1694200}{\textbf{16} 1719}},
    year = {(1973)},
}



@article{Idomura2021,
    author = {Idomura,Y.  and Obrejan,K.  and Asahi,Y.  and Honda,M. },
    title = {Dynamics of enhanced neoclassical particle transport of tracer impurity ions in ion temperature gradient driven turbulence},
    journal = {Phys. Plasmas},
    volume = {\href{https://doi.org/10.1063/5.0027484}{\textbf{28} 012501}},
    year = {(2021)},
}


@article{Esteve2018,
    author = {D. Estève and others},
    title = {Self-consistent gyrokinetic modeling of neoclassical and turbulent impurity transport},
    journal = {Nucl. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/1741-4326/aa6ebb}{\textbf{58} 036013}},
    year = {(2018)},
}


@article{Donnel2019,
    author = {P. Donnel and others},
    title = {{A multi-species collisional operator for full-F global gyrokinetics codes: Numerical aspects and verification with the GYSELA code}},
    journal = {Comput. Phys. Commun.},
    volume = {\href{https://doi.org/10.1016/j.cpc.2018.08.008}{\textbf{234} 1}},
    year = {(2019)},
}

@article{Stacey2006,
    author = {Stacey,W. M.  and Johnson,R. W.  and Mandrekas,J. },
    title = {{A neoclassical calculation of toroidal rotation profiles and comparison with DIII-D measurements}},
    journal = {Phys. Plasmas},
    volume = {\href{https://doi.org/10.1063/1.2212391}{\textbf{13} 062508}},
    year = {(2006)}
}

@article{Field2011,
    author = {A. R. Field and others},
    title = {{Plasma rotation and transport in MAST spherical tokamak}},
    journal = {Nucl. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/0029-5515/51/6/063006}{\textbf{51} 063006}},
    year = {(2006)}
}

@article{Garbet2010,
    author = {X. Garbet and Y. Idomura and L. Villard and T.H. Watanabe},
    title = {Gyrokinetic simulations of turbulent transport},
    journal = {Nucl. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/0029-5515/50/4/043002}{\textbf{50} 043002}},
    year = {(2010)}
}

@article{Kochl2018,
    author = {F Köchl and others},
    title = {{W transport and accumulation control in the termination phase of JET H-mode discharges and implications for ITER}},
    journal = {Plasma Phys. Control. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/1361-6587/aabf52}{\textbf{60} 074008}},
    year = {(2018)}
}
@article{Neu2009,
    author = {R. Neu and others},
    title = {{Ten years of W programme in ASDEX Upgradeâ€”challenges and conclusions}},
    journal = {Phys. Scr.},
    volume = {\href{https://dx.doi.org/10.1088/0031-8949/2009/T138/014038}{\textbf{T138} 014038}},
    year = {(2009)}
}

@article{Angioni2021,
    author = {C. Angioni},
    title = {Impurity transport in tokamak plasmas, theory, modelling and comparison with experiments},
    journal = {Plasma Phys. Control. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/1361-6587/abfc9a}{\textbf{63} 073001}},
    year = {(2021)}
}

@article{Donnel2019_c,
    author = {P. Donnel and others},
    title = {Neoclassical impurity flux in presence of turbulent generated poloidal asymmetries and pressure anisotropy},
    journal = {Plasma Phys. Control. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/1361-6587/ab04b8}{\textbf{61} 044006}},
    year = {(2021)}
}

@article{Kaufmann2007,
    author = {M. Kaufmann and R. Neu},
    title = {Tungsten as first wall material in fusion devices},
    journal = {Fusion Eng. Des.},
    volume = {\href{https://doi.org/10.1016/j.fusengdes.2007.03.045}{\textbf{82} 521}},
    year = {(2007)}
}

@article{Waltz1990,
    author = {Waltz, R. E. and DeBoo, J. C. and Rosenbluth, M. N.},
    title = {Magnetic-field scaling of dimensionally similar tokamak discharges},
    journal = {Phys. Rev. Lett.},
    volume = {\href{https://doi.org/10.1103/PhysRevLett.65.2390}{\textbf{65} 2390}},
    year = {(1990)}
}

@article{Field2023,
    author = {A.R. Field and others},
    title = {{Peripheral temperature gradient screening of high-Z impurities in optimised ‘hybrid’ scenario H-mode plasmas in JET-ILW}},
    journal = {Nucl. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/1741-4326/aca54e}{\textbf{63} 016028}},
    year = {(2023)}
}

@article{Fajardo2023,
    author = {D. Fajardo and others},
    title = {Analytical model for the combined effects of rotation and collisionality on neoclassical impurity transport},
    journal = {Plasma Phys. Control. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/1361-6587/acb0fc}{\textbf{65} 035021}},
    year = {(2023)}
}

@article{Belli2012,
    author = {E. A. Belli and J. Candy},
    title = {{Full linearized Fokker–Planck collisions in neoclassical transport simulations}},
    journal = {Plasma Phys. Control. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/0741-3335/54/1/015015}{\textbf{54} 015015}},
    year = {(2011)}
}

@article{Strugarek2011,
  title = {Unraveling Quasiperiodic Relaxations of Transport Barriers with Gyrokinetic Simulations of Tokamak Plasmas},
  author = {Strugarek, A. and others},
  journal = {Phys. Rev. Lett.},
  volume = {\href{https://dx.doi.org/10.1103/PhysRevLett.111.145001}{\textbf{111} 145001}},
  year = {(2011)}
}

@article{Bucalossi2022,
    author = {J. Bucalossi and others},
    title = {{Operating a full tungsten actively cooled tokamak: overview of WEST first phase of operation}},
    journal = {Nucl. Fusion},
    volume = {\href{https://dx.doi.org/10.1088/1741-4326/ac2525}{\textbf{62} 042007}},
    year = {(2022)}
}

